Who is the Real Hero? Measuring Developer Contribution via Multi-dimensional Data Integration

Proper incentives are important for motivating developers in open-source communities, which is crucial for maintaining the development of open-source software healthy. To provide such incentives, an accurate and objective developer contribution measurement method is needed. However, existing methods rely heavily on manual peer review, lacking objectivity and transparency. The metrics of some automated works about effort estimation use only syntax-level or even text-level information, such as changed lines of code, which lack robustness. Furthermore, some works about identifying core developers provide only a qualitative understanding without a quantitative score or have some project-specific parameters, which makes them not practical in real-world projects. To this end, we propose CValue, a multidimensional information fusion-based approach to measure developer contributions. CValue extracts both syntax and semantic information from the source code changes in four dimensions: modification amount, understandability, inter-function and intra-function impact of modification. It fuses the information to produce the contribution score for each of the commits in the projects. Experimental results show that CValue outperforms other approaches by 19.59% on 10 real-world projects with manually labeled ground truth. We validated and proved that the performance of CValue, which takes 83.39 seconds per commit, is acceptable to be applied in real-world projects. Furthermore, we performed a large-scale experiment on 174 projects and detected 2,282 developers having inflated commits. Of these, 2,050 developers did not make any syntax contribution; and 103 were identified as bots.

==> texs/data.tex <==
\section{Data Availability}

The data and the detailed instruction on how to access the data are published on the anonymous website \url{https://sites.google.com/view/fse23contributionmeasurement}.



==> texs/discussion.tex <==
\section{Discussion}

\subsection{Robustness Analysis}
% add a starting
Our scheme is intended to accurately recognize and motivate developers, and an inappropriate calculation scheme can undermine developer motivation. 
Therefore, it is crucial to prevent reputation-seeker from obtaining relatively high scores for minimal effort. 
In this section, we will discuss potential attacks on this calculation scheme, where individuals may try to obtain higher scores using simple modifications, and how our approach can mitigate such attacks.
% This part will discuss how this calculation method defends against attacks from each aspect.

% \td{LACK A DETAILED EXPLANATION}
% The first is an attack against the amount of AST modification, a common problem in all LoC-based or AST-based computation methods. 
% There is no way to know whether the modification is meaningful by the AST modification amount. 
% To address this problem, our approach has three mitigations: 
% 1) Giving different weights to different types of AST nodes, e.g., changes that only modify variable names, will be ignored in our proposed method, whose detail can be found in Section \ref{sec:refine}. 
% 2) We used a blacklist to block the modification of a series of statements, such as logging and printing to standard output. 
% 3) A large amount of modified AST code must be located where it may be executed and is a relatively important location. 
% Otherwise, such a modification will receive a low importance score, which prevents developers from adding a large amount of code to functions that will not be executed and getting a high score.
The first is an attack about the amount of AST modification, a common problem in all LoC-based or AST-based computation methods. 
These methods cannot determine if the modification is meaningful by simply looking at the amount of AST modification. 
To address this problem, our approach includes the following mitigations:
1) Assigning different weights to different types of AST nodes. 
For example, changes that only modify variable names will be ignored in our proposed method, as detailed in Section \ref{sec:refine}.
2) Using a blacklist to ignore the modification of a series of statements, such as logging and printing to standard output.
3) A large amount of modified AST code should locate in a relatively core location that may be executed. 
Otherwise, such modification will receive a lower inter-function impact score, which prevents developers from adding a large amount of code to functions that will not be executed and getting a high score.

Recent studies have shown that modern AST mapping techniques such as GumTree~\cite{gumtree}, MTDiff~\cite{dotzler2016move}, and IJM~\cite{frick2018generating} have inaccuracies ranging from $20\%$ to $29\%$, $25\%$ to $36\%$, and $21\%$ to $30\%$ respectively~\cite{fan2021differential}. 
% These inaccuracies occur because small changes to code can result in significant differences in the AST. 
Our approach used GumTree, which has relatively high accuracy among the three techniques. 
However, since no AST mapping algorithm has $100\%$ accuracy, which may affect the robustness and accuracy of \tool.

% The second is the complexity metric. 
% Since all complexity metrics were subjected to Box-Cox transformation and adjusted for mean and standard deviation, assuming that the data satisfy a normal distribution with a mean of $1$ and a standard deviation of $\frac{1}{3}$, to raise a single metric from $1$ to $2$ requires that its value for the specific metric exceeds that of $99.85\%$ of the rest of the sample. 
% It is challenging to complete the attack from the perspective of complexity metrics.
The second aspect is the complexity metric. 
Since all complexity metrics have been subjected to the Box-Cox transformation and adjusted for the mean and standard deviation, assuming the data follows a normal distribution with a mean of 1 and a standard deviation of $\frac{1}{3}$, to raise a single metric from 1 to 2, the value for that specific metric would have to exceed that of 99.85\% of the rest of the sample. 
This makes it difficult to attack the complexity metrics.

% The third point is the attack on the consideration of the integrity of the project. 
% Since the integrity concern is calculated from the call graph by a Pagerank-like algorithm with backward propagation, it is not easy to raise the score of a given function. 
% If the score needs to be raised, the function needs to be added to the core logic of the project, and such a modification has a considerable cost.
The third aspect is an attack on the inter-function impact of changes of the project. 
Since the inter-function impact is calculated from the call graph by a Pagerank-like algorithm with backward propagation, it would be difficult to raise the score of a given function. 
To raise the score, the function should be integrated into the core logic of the project, which would require significant modifications, making it a costly attack.

% Finally, an attack on the affected range within a function is difficult to defend against, as it is easy to get a significant value by adding some useless code. 
% A more fine-grained semantic analysis needs to be introduced to solve this problem. 
% However, as with the attacks against AST modifications, the mitigation measures mentioned above also apply to the challenge in this section.
Finally, an attack on the intra-function impact range within a function is difficult to defend against, as it can be easy to artificially inflate the value by adding unnecessary code. 
To address this problem, a more fine-grained semantic analysis would be needed. 
However, similar to the attacks against AST modifications, the mitigation measures mentioned above, such as the use of a blacklist, would also apply to this challenge.

% \subsection{AST Mapping Algorithm}

% % The approach proposed in this paper is based on the degree of change in the AST and incorporates the numerous concerns throughout development to produce a value to measure the contribution of developers. However, modern AST mapping techniques like GumTree~\cite{gumtree}, MTDiff~\cite{dotzler2016move}, and IJM~\cite{frick2018generating} were discovered by Fan et al~\cite{fan2021differential}. to have $20\%$–$29\%$, $25\%$–$36\%$, and $21\%$–$30\%$ inaccurate mappings, respectively. The AST mapping algorithm is capable of receiving specific modifications. A tiny change causes a great difference in the AST. Our approach uses GumTree, which has relatively high accuracy among the three techniques, to mitigate this threat. However, since there is no AST mapping algorithm with $100\%$ accuracy, this attack can only be mitigated but not eradicated.
% The approach presented in this paper is based on the degree of change in the Abstract Syntax Tree (AST) and takes into account various factors to calculate a value that measures the contribution of developers. 
% However, recent studies have shown that modern AST mapping techniques such as GumTree~\cite{gumtree}, MTDiff~\cite{dotzler2016move}, and IJM~\cite{frick2018generating} have inaccuracies ranging from $20\%$ to $29\%$, $25\%$ to $36\%$, and $21\%$ to $30\%$ respectively~\cite{fan2021differential}. 
% These inaccuracies occur because small changes to code can result in significant differences in the AST. 
% Our approach used GumTree, which has relatively high accuracy among the three techniques. 
% However, since no AST mapping algorithm has $100\%$ accuracy, which may affect the robustness and accuracy of \tool.

% \subsection{Impact Range}

% % The proposed method uses Data Dependence Graph (DDG) to detect the impact of changed code. Considering the performance of the software, we are unable to generate a global DDG. Therefore, we cannot predict whether a certain method call of an object will result in modification on the object and hence affect the use of this object in context. This is a typical issue with logging, as logger.info() has no effect on subsequent uses of the logger object. In this approach, we employ a blacklisting mechanism to prohibit certain sorts of objects, assuming that some of its functions will not result in the modification of the object itself. Other objects and methods that, by default, modify the object and so influence its context.
% The proposed method uses Data Dependence Graph (DDG) to determine the inter-function consideration of changing a code segment. 
% However, due to performance constraints, we are unable to generate a global DDG. 
% As a result, it is not possible to predict whether a particular method call on an object will result in modifications to the object and thus affect its use in the context. 
% This is a common issue with logging, as the logger.info() method does not affect subsequent uses of the logger object. 
% To address this issue, we employ a blacklisting mechanism to prohibit certain types of objects, assuming that some of their functions will not result in modifications to the object itself. 
% Other objects and methods, by default, modify the object and thus impact its context.

\subsection{Threats to Validity}

% In Experiment 1 of RQ1, we compare the accuracy of several schemes compared to manually labeled data. 
% There are two threats here. 
% First, the developers who annotated data have not been involved in the development of the projects they annotate. 
% This eliminates any bias they may have towards other developers but also leads to the fact that they may not always truly understand the content and difficulty of the modifications. 
% Second, in Experiment 2 of RQ1, we found that what developers focus on during development and what people who annotate data focus on do not match. 
% Thus manually annotated data may not always represent exactly the right results. 
% These two points can threaten the accuracy of Experiment 1 of RQ1.
In the first experiment of RQ1, where we compare the accuracy of several schemes to manually labeled data, the manully labelled data may be not accurate enough. 
First, the individuals who annotated the data were not involved in the development of the projects they were annotating, which eliminates potential bias but may also lead to a lack of understanding of the content and the difficulty of the modifications. 
Second, developers do not always have the same focus when writing code and reviewing code. 
The views of reviewers of the revisions do not always accurately reflect what the developers were thinking.
These two factors could potentially compromise the accuracy of RQ1.





==> texs/introduction.bak.tex <==
\section{Introduction}

% TODO: Why we need to find core developers
In modern software development, both in companies and open-source communities, collaboration among developers has played an irreplaceable part~\cite{fowler2001agile}. 
In a project, some developers may make more contributions than others and the achievement of the project may strongly depend on these developers. 
As a team leader or project manager, it is important to find these core developers in the group. 
A proper evaluation method can motivate developers, while on the contrary, an approach that is subjective or wrong can be counterproductive. 
Therefore, an objective and sound method is desired to measure the contribution of each developer of the project and to find the core members of the development team~\cite{shull2007guide,herbsleb2003formulation}.

% TODO: Why we need a more objective method
In the "onion" model proposed by Nakakoji et al.~\cite{nakakoji2002evolution}, people involved in the community of open-source software are divided into eight different roles. 
In this model, the frequency of contribution is used to determine whether a developer is peripheral or active. 
It also uses the time since the developer joined the project and the amount of contribution to determine whether a developer is active or core.
There do not exist clear boundaries among periphery developers, active developers, and core developers.

% TODO: Existing methods
There are mainly two kinds of methods to distinguish the core developers from the community, which are count-based methods and network-based methods. 
Count-based methods only measure simple metrics extracted from code change. And use a threshold to classify developers into different categories. 
For example, in the method proposed by Mockus et al.~\cite{mockus2002two}, only the number of lines of code committed by each developer is used for classification. 
In the method proposed by Bella et al.~\cite{di2013multivariate}, multi-variables including lines of code, the number of commits, complexity, comment modifications, and structural and non-structural changes are counted for classification.
As mentioned by Jergensen et al.~\cite{jergensen2011onion}, only counting their activity, such as the number of codes added, can not show their role correctly. 
The interaction of existing code and other developers should be taken into account.
To avoid the defects in count-based methods, Joblin et al.~\cite{joblin_classifying_2017} proposed a network-based approach. 
In this approach, an E-mail network and a version-control-system network are used to analyze the interaction among different developers and the cooperation when committing modifications to the project.
As analyzed by Joblin et al., the results of these two kinds of methods are mostly consistent, although the network-based method agrees more with developer perception than count-based ones.

% TODO: Existing methods
In addition, there are also activity-based role detection methods. Cheng et al.~\cite{cheng2019activity} used four categories of metrics, including code contribution, opinion contribution, network (issues and pull requests), and administrations. 
Izquierdo et al.~\cite{canovas2022analysis} classified people in the community into different roles based on non-code interaction, including comments, issues, pull requests, and commits. 
{\c{C}}etin et al.~\cite{ccetin2022analyzing} use the change history of each file to find the corresponding developer who should be responsible. And they divide the developers in the community into three roles, which are Jacks, Mavens, and Connectors.

% TODO: There are mainly three types of metrics, code change, non-code change, and social activity.
All of the existing methods consider three aspects of information, which are code changes, non-code changes, and social activities. 
Code changes are the changes made to the source code, which directly affect the functionality of the project.
Non-code changes affect other files in the project, including build scripts, documentation, and resource files. 
These changes do not directly affect the operation of the program but are also relevant to development.
Social activities are interactions among developers, whose common forms are creating or commenting on issues, pull requests, reviewing code, etc.
Among these three types of information, social activities are difficult to do objectively and comprehensively quantitative analysis. 
Similarly, it is difficult to do a sound quantitative analysis of non-code changes since non-code changes require corresponding domain knowledge to understand the content of the changes.

% TODO: The metrics used in the existing method are not able to cover the problem.
For metrics used to analyze code changes in previous works only focus on syntax-level or even text-level changes. 
For example, Robles et al.~\cite{robles2009evolution} uses the frequency of committing code in a certain period to find the core team, and Bella et al.~\cite{di2013multivariate} uses the number of lines of code, the number of files, complexity (McCabe cyclomatic complexity~\cite{mccabe1976complexity}) and structure/non-structure modifications, etc. to classify developers into different roles.
However, syntax-level or even text-level changes do not accurately reflect the developer's contribution to the project's functionality. 
For example, formatting code does not require any knowledge of the project and does not make improvements to project functionality, but can produce a large number of text-level changes.
% TODO: The existing metrics only include syntax-level change, we should cover semantic-level change.
In addition, these metrics do not consider the correlation between the changed parts and the whole project, which is important for developers to understand the project and make proper modifications.
Therefore, we need a semantic-level analysis method based on the code change to measure how much each developer contributes to the project functionality and find the core developers.
Extracting and analyzing semantic-level information will lead to performance degradation and the method must strike a reasonable balance between accuracy and time consumption.

% TODO: What we do
To this end, we propose \tool, which is an integration of code-based multi-dimensional features to address the challenges mentioned above. 
It leverages four types of information to assess the code changes in different aspects and produce a comprehensive score to measure the extent to which the developer contributes to the functionality of the project.
First, \tool uses AST differences to measure the syntax-level changes in code, and exclude some non-semantic change patterns like changing the name of variables.
Second, \tool considers the complexity metrics, which include cyclomatic complexity, lines of code, Halstead volume~\cite{halstead1977elements}, and percentage of comment to measure effort to understand the existing code.
Third, a call graph is built, and the position of the changed code segment in the call graph is used to determine the importance of the changed code, which measures the interaction with existing code.
Fourth, \tool traces the  data flow and control flow of the variables involved in the change, aiming the range of context that should be considered by developers when making modifications to the code segment.
In the end, \tool integrates information from these four aspects and provides a more comprehensive view of the change from code level

% TODO: Contribution
To evaluate \tool, we manually labeled 1398 commits on 10 popular projects under Google OSS-Fuzz project~\cite{oss-fuzz} to construct the ground truth. The experimental result shows that \tool outperforms the baseline methods with the spearman correlation of $19.59\%$. Moreover, future analysis has shown that \tool produces a more reasonable assessment than human-labeled ground truth on 1398 commits. On the given project, the average time spent on each commit during \tool analysis was 68.24 seconds on average with a maximum of 121.04 seconds.

In this paper, we made the following contribution:
\begin{enumerate}
    \item We produce \tool, a framework to quantify the contribution made by developers in code commits.
    \item We build an incremental dependency extraction tool, which optimized the time cost for analysis on git repositories.
    \item We conduct an empirical study with \tool on 276 open source projects and found 3155 developers with significant gaps in their number of commits and contribution to the functionality of the project.
\end{enumerate}

